Scam Pandemic: How Attackers Exploit Public Fear through Phishing

As the COVID-19 pandemic started triggering widespread lockdowns across the globe, cybercriminals did not hesitate to take advantage of users' increased usage of the Internet and their reliance on it. In this paper, we carry out a comprehensive measurement study of online social engineering attacks in the early months of the pandemic. By collecting, synthesizing, and analyzing DNS records, TLS certificates, phishing URLs, phishing website source code, phishing emails, web traffic to phishing websites, news articles, and government announcements, we track trends of phishing activity between January and May 2020 and seek to understand the key implications of the underlying trends. We find that phishing attack traffic in March and April 2020 skyrocketed up to 220\% of its pre-COVID-19 rate, far exceeding typical seasonal spikes. Attackers exploited victims' uncertainty and fear related to the pandemic through a variety of highly targeted scams, including emerging scam types against which current defenses are not sufficient as well as traditional phishing which outpaced the ecosystem's collective response.

==> Makefile <==
DOC ?= main.tex 
#$(DOC).tex
DIFF ?= HEAD^
PDFLATEX = pdflatex 
BIBTEX = bibtex
RERUN = "(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
TARDIR = $(DOC:.tex=-src)
IMG_SRCS = $(wildcard figures/*-source.pdf)
IMG_OBJS = $(patsubst %-source.pdf,%.eps,$(IMG_SRCS))

ALL_TEX_FILES = $(shell find . -type f -name '*.tex')
BIB_FILES = $(wildcard *.bib)

.PHONY: pdf clean

pdf: images $(DOC:.tex=.pdf)

all: pdf

%.pdf: %.tex *.tex $(BIB_FILES) $(IMG_OBJS) $(ALL_TEX_FILES)
	$(eval DOC_BASE := $(GENS)$(shell basename $@ .pdf))
	rm -f $(DOC_BASE).bbl
	${PDFLATEX} $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(PDFLATEX) $<) ; true
	egrep -i "(Reference|Citation).*undefined" $*.log ; true
#	dvips -o $(DOC_BASE).ps -t letter $(DOC_BASE).dvi
#	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $(DOC_BASE).ps

watch:
	make; fswatch -0 `find . -name "*.tex" -o -name "*.bib"` | xargs -0 -n1 make all

diff:
	@bin/diff.sh $(DIFF)

clean:
	find . -name "*.aux" | xargs rm -f
	find . -name "*.log" | xargs rm -f
	find . -name "*.out" | xargs rm -f
	find . -name "*.cut" | xargs rm -f
	find . -name "*.upa" | xargs rm -f
	find . -name "*.upb" | xargs rm -f
	find . -name "*.gz"  | xargs rm -f
	@\rm -f \
        $(DOC:.tex=.dvi) \
        $(DOC:.tex=.pdf) \
        $(DOC:.tex=.ps)  \
        $(DOC:.tex=.bbl) \
        $(DOC:.tex=.blg) \
        $(DOC:.tex=.lof) \
        $(DOC:.tex=.lot) \
        $(DOC:.tex=.loc) \
        $(DOC:.tex=.lol) \
	$(DOC:.tex=-src.tar.gz)

images: $(IMG_OBJS)

%.eps: %-source.pdf
	pdftops -eps $< $(<:-source.pdf=.eps)

veryclean: clean
	@\rm -f *~ *.log
	@\rm -f figs/*.pdf

tar: pdf
	@test -d $(TARDIR) || mkdir $(TARDIR)
	@cp Makefile *.{tex,bib,bst,cls} $(TARDIR)
	@tar cz $(TARDIR) > $(TARDIR).tar.gz
	@rm -rf $(TARDIR)


==> __analysis_underground.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.5\linewidth}
        \centering
            \includegraphics[width=\textwidth]{figs/thread_time.pdf}%
        \caption{Thread}
        \label{fig:thread_time}
    \end{subfigure}
    ~
    \begin{subfigure}{0.5\linewidth}
        \centering
            \includegraphics[width=\textwidth]{figs/post_time.pdf}
        \caption{Post}
        \label{fig:post_time}
    \end{subfigure}
    
    \caption{Number of threads/posts over the time}
    \label{fig:thread_post_time}

\end{figure}

\subsection{COVID-19 in Underground Forums}
\label{ss:undermarket}
As underground forums have been the redezvous sites for cybercriminals, we studied two underground forums to understand their members' activities about the COVID-19. We developed crawlers to collect COVID-19 related data, by searching keywords \textit{``coronavirus'', ``2019ncov'', ``covid''}, and \textit{``corona virus''}, from two underground forums: \emph{Nulled.to} and \emph{Cracked.to}, which are popular underground forums having more than 2,800,000 and 1,100,000 registered members respectively. After applying our keywords, we find that 2,913 members engaging in 144 threads from Jan 25, 2020 to May 6, 2020 discuss coronavirus related content in 3,530 posts. 

There are two main questions that we like to answer: (1) Has the coronavirus become a popular topic in underground forums? (2) What do members discuss about coronavirus?

\noindent\textbf{Popularity.} To understand the popularity of the coronavirus discussion, we count the number of threads and posts within one week sliding window because they are indicative of new discussion instances and members' activities. 
As shown in Figure~\ref{fig:thread_post_time}, the growth patterns of threads and posts are similar and start to increase since Feb 15, 2020. %We both the number of threads and posts  grows after  Feb 15, 2020. 
We noticed a significant peak on April 15, and conducted the thread analysis finding that 58.3\% of the new threads are started by the same vendor who joined the forum on Feb 24, 2020 for selling different compromised accounts, such as cracked Disney premium accounts, Brazers premium accounts, etc. 

\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{figs/content_time.pdf}
    \caption{Different contents over the time in underground forums.}
    \label{fig:content_time}
\end{figure}

\noindent\textbf{Discussion.} We manually analyzed all of these 144 threads and found out that members in underground forums mainly discuss four topics categorized as (1) virus (e.g., what the corona virus is); (2) money (e.g., how to make money during coronavirus time); (3) hacking (e.g., hacking services or scripts); and (4) account (e.g., compromised account trading).
The details of the categories and main topic types in each category are shown in Table~\ref{tab:content_category}. 
We notice that there are five types of accounts are trading in underground forums with mentioning coronavirus in the advertising, which are game accounts, VPN accounts, video account (Netflix), music site account (Spotify), and porn site accounts.  

\begin{table}[t]
\centering
\footnotesize
    \begin{tabular}{crr}
    \toprule
    \multicolumn{1}{c}{\textbf{Content Category}} & \textbf{Sub-category} & \textbf{\% of discussions}\\
    \midrule
    
    \multirow{2}{*}{Virus} & Virus\_general & 93.8\%\\
     & Virus\_protection & 6.2\%\\
     \cdashline{1-3}[0.8pt/2pt]
     
     \multirow{5}{*}{Account} & Account\_game & 37.7\%\\
     & Account\_VPN & 24.7\%\\
     & Account\_video & 18.2\%\\
     & Account\_music & 10.4\%\\
     & Account\_porn & 9.1\%\\
     \cdashline{1-3}[0.8pt/2pt]
     
   \multirow{2}{*}{Money} & Money\_general & 45.5\%\\
    & Money\_ewhoring & 54.5\%\\
    \cdashline{1-3}[0.8pt/2pt]
    
    \multirow{3}{*}{Hacking} & Hacking\_crack & 40.0\%\\
    & Hacking\_accountchecker & 40.0\%\\
    & Hacking\_phishing & 20.0\%\\
    
    \bottomrule
    \end{tabular}
\caption{Coronavirus-related discussion in underground forums. }
\label{tab:content_category}
\end{table}


As depicted in Figure~\ref{fig:content_time}, at the beginning of the period people mainly discuss the coronavirus, while changing to compromised accounts since April 1, 2020. 


% underground communities ? [Eric]
    %% underground forum metrics
    %% content of corona threats
    %% examples of malware
    %% uptick in cracked accounts **
    %% dark web case studies, differences between underground and dark web, or time line

==> __communications.tex <==
\subsection{Communications}
\label{ss:comms}
To study the effect of COVID-19 pandemic on corona-themed social engineering attacks, the first step is to examine how the government and news outlets are reacting toward such attacks. This motivates us to study the reported news regarding this matter. Hence, we collect daily reported news starting from January 2020 alongside official governmental announcements. 

% Rapid growth of corona-related social engineering attacks, motivate us to study the reported news regarding this matter. Hence, we collect daily reported news starting from January 2020 alongside official governmental announcements. 
%After looking into collected data we notice the first news about corona-related scam was released on StartDate by Website.
We provide a scheme of the growing process of news and government announcements about corona-related scams through this dataset. 
% \textcolor{red}
\autoref{fig:GovernmenandNews} shows the CDF of coronavirus government and press news. This figure demonstrates that the number of corona-related scam news is growing from the beginning of this pandemic in January 2020. The non-governmental news began to reference to corona-virus scam in January $30^{th}$, stating that several campains are sending corona-related emails containing malware. Moreover, the first government official warnings about corona-virus scams started from February $1^{st}$ warning people about cybercriminals trying to leverage COVID-19 situation. Most of these announcements include detailed guidance for people how to protect themselves from these frauds. 

After looking into the results, we notice rapid growth of news regarding the corona-related social engineering attacks. This conclusion reveals the need for an extensive analysis on how the COVID-19 pandemic has affected the internet infrastructure. 
\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{figs/NvsGA.pdf}
    \caption{The number of Corona-virus related scams news and government announcements during time.}
    \label{fig:GovernmenandNews}
\end{figure}

% The number of average news per day is X, and its peak is X in XDate. The news began to reference to corona-virus scam in X date.
% The provided CDF shows the speed of news coverage growth of corona-related scam.
% Additionally, in figure X We showed the number of government announcements about corona-related scams starting from January 2020. This overview demonstrates the peak of these announcements or warnings is in XDate.
%The first official warnings about corona-virus scams started from xdate. Most(maybe the I should calculate the exact number) of these announcements include detailed guidance for people how to protect them selves from these frauds.
%is the CDF on the number of announcements/warnings related to coronavirus on government websites:

% communications [Marzieh/Rana]
    %% news volume / CDF
    %% government (industry) covid scam announcement timeline
    %% law enforcement action timelin

==> ack.tex <==
\section{Acknowledgment}
\label{s:ack}


==> summary.tex <==
\subsection{Synthesizing Results of Measurement}
\label{ss:summary1}
Analyzing the collected dataset indicates the large number of domains may confuse Internet users as it makes it hard for them to distinguish fraud websites among the legitimate ones.
Also, it suggests that the government started to warn users concerning corona-related phishing scams after victims reported significant number of attacks. 
The low number of intersections between the collected DNS records and anti-phishing entities' blacklists, alongside with the FTC report~\cite{scamreports} indicates that a significant amount of registered domains have been used for other non-phishing attacks. 
To find out what attackers are exploiting, we analyzed phishing websites' contents. 
The results indicate that the attackers leverage users' needs to lure victims. 
For example, they use users' fear on PPE shortage to deceive them. 
Finally, by monitoring corona-related discussions on underground forums, we suspect that the attackers' activities increase after they successfully carry on their attacks. The activities include posting about stolen accounts. 

%Moreover, our findings through analyzing the the progression of phishing websites, reveals that the number of victims decreases after the government made several announcements regarding corona-related social engineering attacks. 
%We performed a series of measurements to seek answer to two main questions: (1) what are attackers exploiting, and (2) how they are taking advantage of the COVID-19 situation. As a preliminary step in our study, we collected news about corona-themed phishing scams, from both news outlets and government officials. By analyzing the news, we found that the number of warnings about this matter has been on an increase. To answer the so-called questions, then we collect DNS records, web traffic, CT logs, and phishing URLs. and the attackers are leveraging people's fear to lay traps. Furthermore, analyzing the web crawler data, and threat intelligence data allows us to categorize the corona-themed phishing websites into different categories such as donation themed phishing and free shipping phishing websites. Additionally, studying discussions in two popular underground forums indicates that threads and posts related to corona have been increasing. The users in these forums mainly discuss the corona virus itself, how to make money during the corona pandemic, hacking, and stolen accounts. Finally, by scrutinizing the reported phishing emails and web crawled data using the Golden Hour approach, we observe an increase in the amount of phishing emails. 

